MERaLiON-AudioLLM: Bridging Audio and Language with Large Language Models

We introduce MERaLiON-AudioLLM (Multimodal Empathetic Reasoning and Learning in One Network), the first speech-text model tailored for Singapore's multilingual and multicultural landscape. Developed under the National Large Language Models Funding Initiative, Singapore, MERaLiON-AudioLLM integrates advanced speech and text processing to address the diverse linguistic nuances of local accents and dialects, enhancing accessibility and usability in complex, multilingual environments. Our results demonstrate improvements in both speech recognition and task-specific understanding, positioning MERaLiON-AudioLLM as a pioneering solution for region specific AI applications. We envision this release to set a precedent for future models designed to address localised linguistic and cultural contexts in a global framework.

==> fig-tree.tex <==
\begin{forest}
  for tree={
  grow=east,
  reversed=true,
  anchor=base west,
  parent anchor=east,
  child anchor=west,
  base=left,
  font=\small,
  rectangle,
  draw,
  rounded corners,align=left,
  minimum width=2.5em,
  inner xsep=4pt,
  inner ysep=1pt,
  },
  where level=1{text width=5em,fill=blue!10}{},
  where level=2{text width=5em,font=\footnotesize,fill=pink!30}{},
  where level=3{font=\footnotesize,yshift=0.26pt,fill=yellow!20}{},
  [\textbf{AudioBench} \\ Benchmark for AudioLLMs,fill=green!20
        [Automatic Speech Recognition (ASR),text width=13em
            [LibriSpeech-Clean~\cite{panayotov2015librispeech},text width=14.5em]
            [LibriSpeech-Other~\cite{panayotov2015librispeech},text width=14.5em]
            [CommonVoice~\cite{ardila-etal-2020-common},text width=13.5em]
            [PeoplesSpeech~\cite{galvez2021people},text width=13.5em]
            [Earning-21~\cite{del2021earnings},text width=13.5em]
            [Earning-22~\cite{del2022earnings},text width=13.5em]
            [GigaSpeech~\cite{chen2021gigaspeech},text width=13.5em]
            [Tedium3~\cite{rousseau2012ted},text width=13.5em]
            [Tedium3-Longform~\cite{rousseau2012ted},text width=15em]
        ]
        [Speech Question Answering (SQA),text width=12em
            [CN-College-Listen~\cite{hu2024wavllm},text width=18em]
            [SLUE-P2-SQA5~\cite{shon2022slue},text width=13.5em]
            [DREAM-TTS~\cite{sun2019dream},text width=13.5em]
            [Public-SG-SpeechQA,text width=13.5em]
        ]
        [Audio Question Answering (AQA),text width=12em          
            [Clotho-AQA~\cite{lipping2022clotho},text width=13.5em]
            [WavCaps-QA~\cite{mei2023wavcaps},text width=13.5em]
            [AudioCaps-QA~\cite{audiocaps},text width=13.5em]
        ]
        [Emotion Recognition (ER),text width=9em               
            [IEMOCAP-Emotion~\cite{busso2008iemocap},text width=13.5em]
            [MELD-Sentiment~\cite{poria-etal-2019-meld},text width=13.5em]
            [MELD-Emotion~\cite{poria-etal-2019-meld},text width=13.5em]
        ]
        [Speech Instruction (SI),text width=8em              
            [OpenHermes-Audio~\cite{OpenHermes},text width=15em]
            [ALPACA-Audio~\cite{alpaca},text width=15em]
        ]
        [Audio Captioning (AC),text width=8em              
            [WavCaps~\cite{mei2023wavcaps},text width=13.5em]
            [AudioCaps~\cite{audiocaps},text width=13.5em]
        ]
        [Accent Recognition (AR),text width=8.5em              
        [VoxCeleb-Accent~\cite{nagrani2017voxceleb},text width=13.5em]
        ]
        [Gender Recognition (GR),text width=8.5em              
            [VoxCeleb-Gender~\cite{nagrani2017voxceleb},text width=13.5em]
            [IEMOCAP-Gender~\cite{busso2008iemocap},text width=13.5em]
        ]
        [Future Tasks,text width=7em              
            [Audio Generation Tasks,text width=9em 
                [Text-to-Speech (TTS)] 
                [Voice Conversion (VC)]
                [Speech Segmentation (SS)]
            ]
            [Multilingual Understanding,text width=10em
                [Speech Translation (ST) \& others.]]
            [Multiple Audio Understanding,text width=10.5em
                [Speaker Verification (SV) \& others.]
            ]
            [etc.,text width=5em]
        ]
    ]
\end{forest}

==> sections/analyses.tex <==
\section{Analyses}
\subsection{1. What should we fine-tune?}

\subsection{1. Normalize ASR inputs?}

\subsection{2. Melspectrogram augmentation}
\subsection{1. IF Eval}

==> sections/discussions.tex <==
\section{Discussions}

==> tables/training_datasets.tex <==
\begin{table*}[ht!]

\scriptsize
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{Task} & \textbf{Description} & \textbf{Metric} & \textbf{Dataset} & \textbf{Split}\\ 
\midrule
\multirow{5}{*}{ASR} & \multirow{5}{*}{Automatic Speech Recognition} & \multirow{5}{*}{WER $(\downarrow)$} 
& Common Voice 17 - En & train | dev | test \\
%& & & GigaSpeech & train | dev | test \\
& & & People's Speech & train | dev | test \\
& & & LibriSpeech & train | test \\
& & & National Speech Corpus & train | test \\ \midrule
\multirow{4}{*}{ST} & \multirow{4}{*}{Speech Translation} & \multirow{4}{*}{BLEU $(\uparrow)$}
& CoVoST-2 & train | dev | test \\
& & & Common Voice 17 & train | test \\
%& & & GigaSpeech & train | test \\
& & & People's Speech & train | test \\ \midrule
\multirow{11}{*}{SQA} & \multirow{11}{*}{Spoken Question Answering} & \multirow{11}{*}{LLM-as-a-Judge $(\uparrow)$} 
& Common Voice 17 SQA & train | test \\
& & & DREAM & train | test \\
%& & & GigaSpeech SQA & train | test \\
& & & LibriSpeech SQA & train | test \\
& & & National Speech Corpus SQA & train | test \\
& & & People's Speech SQA & train | test \\
& & & SLUE-SQA-5 & train | test \\
& & & Spoken SQuAD & train | test \\
& & & CN College Entrance English Test & test \\
& & & ODSQA & test \\
& & & Singapore Public Speech SQA & test \\ \midrule
\multirow{1}{*}{DS} & \multirow{1}{*}{Data Summarization} & \multirow{1}{*}{LLM-as-a-Judge $(\uparrow)$} 
& National Speech Corpus & train | test \\ \midrule
\multirow{2}{*}{SI} & \multirow{2}{*}{Speech Instruction} & \multirow{2}{*}{LLM-as-a-Judge $(\uparrow)$} 
& Alpaca-GPT4-TTS & train | test \\
& & & Open Hermes-TTS & train | test \\ \midrule
\multirow{3}{*}{PARA} & \multirow{3}{*}{Paralinguistics} & \multirow{3}{*}{LLM-as-a-Judge $(\uparrow)$} 
& MELD & train | test \\
& & & National Speech Corpus & train | test \\
& & & VoxCeleb1 & train | test \\
\midrule
\multirow{2}{*}{AC} & \multirow{2}{*}{Audio Captioning} & \multirow{2}{*}{LLM-as-a-Judge $(\uparrow)$} 
& AudioCaps & train | test \\
& & & WavCaps & train | test \\ \midrule
\multirow{3}{*}{ASQA} & \multirow{3}{*}{Audio Scene Question Answering} & \multirow{3}{*}{LLM-as-a-Judge $(\uparrow)$} 
& AudioCaps ASQA & train | test \\
& & & Clotho ASQA & train | test \\
& & & WavCaps ASQA & train | test \\
\bottomrule
\end{tabular}
\caption{Summary of training and evaluation tasks and datasets.} 
\label{tab:overall_data_stats}
    
\end{table*}
